Revealing the conformal symmetry of the discrete series scalars in dS${}_2$

On two-dimensional manifolds with nonzero constant Ricci curvature, there exists an infinite sequence of scalar fields with nonzero mass parameter that admit a pair of (anti-)holomorphic currents. After suitably defining the theory in de Sitter space ($\mathrm{dS}_2$), correlation functions of these currents obey global conformal Ward identities. We address the question of how this global conformal symmetry manifests as an action on the scalar field. An essential step is in leveraging an equivalent description of the scalar field in terms of a conformal Killing tensor. Through this, we find a conformal symmetry transformation that acts locally on the conformal Killing tensor, but non-locally on the scalar field. We show that the equation of motion transforms covariantly with respect to these conformal transformations, and further find a traceless stress tensor in both $\mathrm{dS}_2$ and $\mathrm{AdS}_2$, locally defined in terms of the conformal Killing tensor, which generates the global conformal isometry transformations.

==> preambledefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Nick Geiser
% ngeiser@physics.ucla.edu
% last updated 2022/08/02
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppercase calligraphic shorthand via \mathcal
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppercase bold shorthand via \boldsymbol
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bfA}{\boldsymbol{A}}
\newcommand{\bfB}{\boldsymbol{B}}
\newcommand{\bfC}{\boldsymbol{C}}
\newcommand{\bfD}{\boldsymbol{D}}
\newcommand{\bfE}{\boldsymbol{E}}
\newcommand{\bfF}{\boldsymbol{F}}
\newcommand{\bfG}{\boldsymbol{G}}
\newcommand{\bfH}{\boldsymbol{H}}
\newcommand{\bfI}{\boldsymbol{I}}
\newcommand{\bfJ}{\boldsymbol{J}}
\newcommand{\bfK}{\boldsymbol{K}}
\newcommand{\bfL}{\boldsymbol{L}}
\newcommand{\bfM}{\boldsymbol{M}}
\newcommand{\bfN}{\boldsymbol{N}}
\newcommand{\bfO}{\boldsymbol{O}}
\newcommand{\bfP}{\boldsymbol{P}}
\newcommand{\bfQ}{\boldsymbol{Q}}
\newcommand{\bfR}{\boldsymbol{R}}
\newcommand{\bfS}{\boldsymbol{S}}
\newcommand{\bfT}{\boldsymbol{T}}
\newcommand{\bfU}{\boldsymbol{U}}
\newcommand{\bfV}{\boldsymbol{V}}
\newcommand{\bfW}{\boldsymbol{W}}
\newcommand{\bfX}{\boldsymbol{X}}
\newcommand{\bfY}{\boldsymbol{Y}}
\newcommand{\bfZ}{\boldsymbol{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lowercase bold shorthand via \boldsymbol
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bfa}{\boldsymbol{a}}
\newcommand{\bfb}{\boldsymbol{b}}
\newcommand{\bfc}{\boldsymbol{c}}
\newcommand{\bfd}{\boldsymbol{d}}
\newcommand{\bfe}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bfg}{\boldsymbol{g}}
\newcommand{\bfh}{\boldsymbol{h}}
\newcommand{\bfi}{\boldsymbol{i}}
\newcommand{\bfj}{\boldsymbol{j}}
\newcommand{\bfk}{\boldsymbol{k}}
\newcommand{\bfl}{\boldsymbol{l}}
\newcommand{\bfm}{\boldsymbol{m}}
\newcommand{\bfn}{\boldsymbol{n}}
\newcommand{\bfo}{\boldsymbol{o}}
\newcommand{\bfp}{\boldsymbol{p}}
\newcommand{\bfq}{\boldsymbol{q}}
\newcommand{\bfr}{\boldsymbol{r}}
\newcommand{\bfs}{\boldsymbol{s}}
\newcommand{\bft}{\boldsymbol{t}}
\newcommand{\bfu}{\boldsymbol{u}}
\newcommand{\bfv}{\boldsymbol{v}}
\newcommand{\bfw}{\boldsymbol{w}}
\newcommand{\bfx}{\boldsymbol{x}}
\newcommand{\bfy}{\boldsymbol{y}}
\newcommand{\bfz}{\boldsymbol{z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppercase Fraktur shorthand via \mathfrak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mfA}{\mathfrak{A}}
\newcommand{\mfB}{\mathfrak{B}}
\newcommand{\mfC}{\mathfrak{C}}
\newcommand{\mfD}{\mathfrak{D}}
\newcommand{\mfE}{\mathfrak{E}}
\newcommand{\mfF}{\mathfrak{F}}
\newcommand{\mfG}{\mathfrak{G}}
\newcommand{\mfH}{\mathfrak{H}}
\newcommand{\mfI}{\mathfrak{I}}
\newcommand{\mfJ}{\mathfrak{J}}
\newcommand{\mfK}{\mathfrak{K}}
\newcommand{\mfL}{\mathfrak{L}}
\newcommand{\mfM}{\mathfrak{M}}
\newcommand{\mfN}{\mathfrak{N}}
\newcommand{\mfO}{\mathfrak{O}}
\newcommand{\mfP}{\mathfrak{P}}
\newcommand{\mfQ}{\mathfrak{Q}}
\newcommand{\mfR}{\mathfrak{R}}
\newcommand{\mfS}{\mathfrak{S}}
\newcommand{\mfT}{\mathfrak{T}}
\newcommand{\mfU}{\mathfrak{U}}
\newcommand{\mfV}{\mathfrak{V}}
\newcommand{\mfW}{\mathfrak{W}}
\newcommand{\mfX}{\mathfrak{X}}
\newcommand{\mfY}{\mathfrak{Y}}
\newcommand{\mfZ}{\mathfrak{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lowercase Fraktur shorthand via \mathfrak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mfa}{\mathfrak{a}}
\newcommand{\mfb}{\mathfrak{b}}
\newcommand{\mfc}{\mathfrak{c}}
\newcommand{\mfd}{\mathfrak{d}}
\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mff}{\mathfrak{f}}
\newcommand{\mfg}{\mathfrak{g}}
\newcommand{\mfh}{\mathfrak{h}}
\newcommand{\mfi}{\mathfrak{i}}
\newcommand{\mfj}{\mathfrak{j}}
\newcommand{\mfk}{\mathfrak{k}}
\newcommand{\mfl}{\mathfrak{l}}
\newcommand{\mfm}{\mathfrak{m}}
\newcommand{\mfn}{\mathfrak{n}}
\newcommand{\mfo}{\mathfrak{o}}
\newcommand{\mfp}{\mathfrak{p}}
\newcommand{\mfq}{\mathfrak{q}}
\newcommand{\mfr}{\mathfrak{r}}
\newcommand{\mfs}{\mathfrak{s}}
\newcommand{\mft}{\mathfrak{t}}
\newcommand{\mfu}{\mathfrak{u}}
\newcommand{\mfv}{\mathfrak{v}}
\newcommand{\mfw}{\mathfrak{w}}
\newcommand{\mfx}{\mathfrak{x}}
\newcommand{\mfy}{\mathfrak{y}}
\newcommand{\mfz}{\mathfrak{z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppercase blackboard bold (doublestroke) shorthand via \mathbb
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lowercase Greek shorthand
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\g}{\gamma}
\renewcommand{\d}{\delta}
\newcommand{\e}{\varepsilon}
\newcommand{\ve}{\varepsilon}
% \zeta
% \eta
\renewcommand{\th}{\theta}
\newcommand{\vth}{\vartheta}
% \iota
\newcommand{\kap}{\kappa}
\newcommand{\vkap}{\varkappa}
\newcommand{\lam}{\lambda}
% \mu
% \nu
% \xi
% \omicron = o
% \pi
\newcommand{\vpi}{\varpi}
% \rho
\newcommand{\vrho}{\varrho}
\newcommand{\sig}{\sigma}
\newcommand{\vsig}{\varsigma}
% \tau
\newcommand{\ups}{\upsilon}
\newcommand{\f}{\varphi}
\newcommand{\vf}{\varphi}
% \chi
% \psi
\newcommand{\om}{\omega}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppercase Greek shorthand
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \Alpha = A
% \Beta = B
\newcommand{\G}{\Gamma}
\newcommand{\vG}{\varGamma}
\newcommand{\D}{\Delta}
\newcommand{\vD}{\varDelta}
% \Epsilon = E
% \Zeta = Z
% \Eta = H
\newcommand{\Th}{\Theta}
\newcommand{\vTh}{\varTheta}
% \Iota = I
% \Kappa = K
\newcommand{\Lam}{\Lambda}
\newcommand{\vLam}{\varLambda}
% \Mu = M
% \Nu = N
% \Xi
\newcommand{\vXi}{\varXi}
% Omicron = O
% \Pi
\newcommand{\vPi}{\varPi} 
% \Rho = P
\newcommand{\Sig}{\Sigma}
\newcommand{\vSig}{\varSigma}
% \Tau = T
\newcommand{\Ups}{\Upsilon}
\newcommand{\vUps}{\varUpsilon} 
\newcommand{\F}{\Phi} 
\newcommand{\vF}{\varPhi} 
% \Chi = X
% \Psi
\newcommand{\vPsi}{\varPsi}
\newcommand{\Om}{\Omega}
\newcommand{\vOm}{\varOmega}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% delimiter shorthand
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% math
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\p}{\partial}

% 3-argument "thermodynamics" partial derivative
\newcommand{\dthermo}[3]{\left( \frac{\partial #1}{\partial #2} \right)_{#3}}

% math operators
\DeclareMathOperator{\Det}{Det}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator*{\Res}{Res}

% better real and imaginary parts
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}

% floor and ceiling
\newcommand{\floor}[1]{\cramped{\left\lfloor #1 \right\rfloor}}
\newcommand{\ceil}[1]{\cramped{\left\lceil #1 \right\rceil}}

% extendable tilde for asymptotic expressions
\newcommand{\widesim}[2][1.5]{
  \mathrel{\overset{#2}{\scalebox{#1}[1]{$\sim$}}}
}

% small text-style symbols
\newcommand{\tsum}{\textstyle\sum\nolimits}
\newcommand{\tprod}{\textstyle\prod\limits}
\newcommand{\half}{\tfrac{1}{2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% negative phantom space
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\negphantom}[1]{
    \ifmmode\settowidth{\dimen0}{$#1$}
    \else\settowidth{\dimen0}{#1}
    \fi
    \hspace*{-\dimen0}}
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mask: center in box with specified width
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Note to self: rewrite this function using \makebox and \settowidth
\makeatletter
\newcommand{\mask}[2]{{\mathpalette\mask@{{#1}{#2}}}}
\newcommand{\mask@}[2]{\mask@@{#1}#2}
\newcommand{\mask@@}[3]{%
  \settowidth{\dimen@}{$\m@th#1#2$}%
  \makebox[\dimen@]{$\m@th#1#3$}%
}
\makeatother
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Eric D'Hoker's formatting defs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\sm}{\smallskip}
\newcommand{\no}{\nonumber}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% future typesetting projects
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Condense the definitions at top of this document using for-loop.
% Figure out consistent delimiter spacing with \left and \right. I think these commands add some unnecessary white space.
% Find way to consistently reduce space between +, -, etc. in long equations.
% Find way to uniformize vertical spacing in multiline equations.
% Why do the \floor, \ceil, \bmatrix brackets look bigger in JHEP published version of my 2021 paper?


